The 2021 RecSys Challenge Dataset: Fairness is not optional

After the success the RecSys 2020 Challenge, we are describing a novel and bigger dataset that was released in conjunction with the ACM RecSys Challenge 2021. This year's dataset is not only bigger (~ 1B data points, a 5 fold increase), but for the first time it take into consideration fairness aspects of the challenge. Unlike many static datsets, a lot of effort went into making sure that the dataset was synced with the Twitter platform: if a user deleted their content, the same content would be promptly removed from the dataset too. In this paper, we introduce the dataset and challenge, highlighting some of the issues that arise when creating recommender systems at Twitter scale.

==> 01_intro.tex <==
\section{Intro}
Recommender systems play a huge role in modern social media platforms, and this is true for Twitter: when a user logs in, they are presented with a series of Tweets (the Home timeline) that are ranked according to the user's preferences (more on it later). 

Datasets have played a huge role into shaping the development of new techniques, especially deep learning. 
For example, consider the rapid pace of innovations in computer vision that followed by the release of the ImageNet dataset \cite{Deng09imagenet:a}. 
In a similar fashion, the field of natural language processing (NLP) has seen similar improvements since the release of BERT in 2018, followed by ELMo and more recently GPT-3.  As pointed out by \cite{10.1145/3442188.3445922}, there are many issues when training large language models: among others environmental costs and the documented bias that those models carry over from their training data.

At the same time, it seems that recommender systems  have not really reaped the benefits of modern methods and technologies. For example, \cite{10.1145/3383313.3412488} shows how replacing dot-product similarities with multi layer perceptron, does not bring any real advantages – while requiring more time and resources to train and maintain.


% GDL
Of particular interest at Twitter are methods that leverage the emerging field of geometric deep learning, which is synonymous with Graph Neural Networks (GNN)s. These methods are able to fuse relational and content information to perform task specific learning in graphs that may be directed and have multiple heterogenous features and edges types. Such methods have already been successfully applied to recommendation tasks in social media and e-commerce \cite{ying2018graph, zhu2019aligraph, wang2019explainable}.


We believe that increasing the availability of public large scale datasets that are tailored specifically for recommender systems will help foster research. That is why we introduce this challenge – and its accompanying dataset: we hope to bridge the gap between industry practitioners and researchers.


In Section \ref{problem-definition} we formally introduce the task of the  challenge, while explaining the differences between the challenge and Twitter's product usage.
In Section \ref{challenges-at-scale} we closely examine the challenges that come with Twitter scale, while Section \ref{challenge-dataset} describes the challenge's dataset. Finally in Section \ref{challenge} we discuss the 2021 RecSys Challenge in detail, providing details on how submissions are evaluated and the baseline that we provided.



==> 03_challenges.tex <==
\section{Challenges} \label{challenges-at-scale}
In this section, we describe some of the challenges that are very common in recommender systems deployed in industry especially for Twitter's scale.

\subsection{Feature Selection: Social Graph}
While feature selection is a common problem for machine learning practitioners, we would like to specifically focus on the problem of social graph.
On Twitter, users can follow each other. Since the number of unique users is on the order of hundreds of millions, this size poses the problem of how to practically encode this follower / followee relationship. 

If we one-hot encode each user, the feature space would explode in dimension. This design choice will cause all sort of engineering problems: more data is required to avoid overfitting, more hardware is required, and latency might increase (also see Section \ref{latency}).

\subsection{Sampling and label imbalance}
Each day hundreds of millions of Tweets are produced by users all across the world. Ideally, when training a machine learning model, it is possible to use all the available data (after splitting in train/test/validation). In reality, at this scale this is not possible - mostly due to time constrains (more data will require more time, and this more resources to train the model). At the same time, very old data might not be relevant for training purposes, e.g. adding content from 2012 would probably not provide any benefits to a model trained in 2021 (likely the opposite will be true). 

The practitioner  has to make a choice then: specifically how much data is required to train the model and how to sample it. 
In the case of Twitter, there is also a big label imbalance between positive and negative examples. A positive example is a Tweet that the user saw and engaged with, while a negative one is a Tweet that the user saw but decided \emph{not} to engage with. Users tend to engage with a fraction of the Tweets they see. This behavior translates into a strong imbalance between the positive and negative classes. 

\subsection{Latency}\label{latency}
The real-time nature of Twitter makes latency a primary concern. When a user logs in on the platform and requests a new timeline (i.e. a fresh set of Tweets to see on their Home timeline), it is important that the ranking is done in real time and must hold true for all the hundreds of millions of users that refresh their timeline every day. Any model that requires more than a few millisecond to score would be considered too slow and not suitable for production settings. If we had access to a slow but perfect oracle-like model that is able to produce the perfect ranking, we would have no use for it.


\subsection{Intrinsic value of metrics}\label{value-of-metrics}
Ideally the ranking of the Tweets would reflect the readers' preferences, with the most valuable ones being on top. In practice, it is hard to asses the intrinsic value of a piece of content, since the users are not asked to rank or score them (contrast with a movie streaming service where a user can rank each piece of content). While engagement is the industry-standard metric (the hypothesis being that if a person engaged with a Tweet, they found it valuable), it is important to remember that is a proxy-metric, and that in the current settings it is hard to disentangle value from engagements (e.g. \cite{smitha, dylan}).

\subsection{Data shift}
As mentioned earlier, when users log in to Twitter they expect to see content that is both relevant and timely. At the same time the discourse changed very rapidly: events can shift the conversations pretty quickly (e.g. a natural disaster or sports events) and trending topics can change as quickly. On top of that, the same hashtag might be used to mean different things at different times. It is thus vital for a service like Twitter to have models that are constantly trained on fresh data to properly represent the latest status of the platform.
A potential way of mitigating this problem, is to divide the main model in sub-parts (e.g. embeddings) that can be more easily retrained. For Twitter's case see \cite{shiebler2018fighting} for more details.

\subsection{Graph Neural Network Methods}

Overwhelmingly, GNN research deals with graphs and associated features that can be loaded into GPU memory. For large scale applications such as the recommendation systems at Twitter, this is not possible and training must resort to a batching strategy. In computer vision or NLP, samples are usually treated as independent and identically distributed (iid) and parallelising over batches using SGD is a solved problem. This is not the case for graph data where all pairs of nodes are related and batching requires making difficult choices about how to cut the graph. Methods such as graphSAGE/PinSAGE~\cite{hamilton2017inductive, ying2018graph} perform batching by taking a 2-hop neighbourhood~\footnote{in reality even this is too large and only a small fixed number of neighbours at each hop are taken} around each ``training node.'' This approach is highly inefficient compared to full batch training since in each batch the vast majority of nodes are ``feature nodes'' and are not for training. This problem has been addressed by methods that generate subgraphs in which each node is used both as a feature and training node \cite{zeng2019graphsaint, chen2018fastgcn}, but there remains the difficult problem of selecting subgraphs. Some recent methods sidestep this problem by precomputing multihop features \cite{rossi2020sign}, but these tradeoff scalability for expressivity.



==> table.tex <==
\begin{sidewaystable}

\begin{table}[H]
%\resizebox{\linewidth}{!}{
%\begin{tabular}{|>{\Large}c| >{\Large}l | >{\Large}l | >{\Large}l |}
\begin{tabular}{|c| l | l | l |}
\hline
%\multicolumn{1}{|>{\Large}c|}{\textbf{Feature } } & %\multicolumn{1}{>{\Large}c|}{\textbf{Name} } & %\multicolumn{1}{>{\Large}c|}{\textbf{Signature} } & %\multicolumn{1}{>{\Large}c|}{\textbf{Description} } \\
\textbf{Feature } & \textbf{Name} &\textbf{Signature} &\textbf{Description} \\
 \hline
{\multirow{5}{*}{\textbf{User}}} & userId & \textit{string}   & User identifier (hashed) \\
                                     & follower count & \textit{int}                  & Number of followers of the user                                  \\
                                      & following count & \textit{int}                  & Number of accounts this  user is following                        \\
                                       & is verified & \textit{bool}                      & Is the account verified?                                         \\
                                    &  account creation time & \textit{int}  & timestamp of the creation time of the account \\ 
  \hline
{\multirow{7}{*}{\textbf{Tweet}}} &  tweetId & \textit{string}                            & Tweet identifier (hashed)                                                 \\
                                     &  presentMedia & \textit{list[string]}                  & Tab-separated list of media types; media type can be in (Photo, Video, Gif)                                  \\
                                      &  presentLinks & \textit{list[string]}                  & Tab-separated list of links included in the tweet (hashed)                       \\
                                          &  presentDomains & \textit{list[string]}                  & Tab-separated list of domains (e.g. twitter.com) included in the tweet (hashed)   
                           \\           &  tweetType & \textit{string}                     & Tweet type, can be either Retweet, Quote, Reply, or Toplevel                                         \\
                                       & language & \textit{string}  & Identifier corresponding to inferred language of the tweet \\
                                       &  tweet timestamp& \textit{int}                      & Unix timestamp, in seconds of the creation time of the Tweet                                         \\
                                       &  tweet tokens & \textit{list[int]}   & Ordered list of Bert ids corresponding to Bert tokenization of Tweet text \\
                                            &  tweet hashtags & \textit{list[string]}   & Tab-separated list of hashtags present in the tweet \\
\hline                                      
\multirow{5}{*}{\textbf{Engagement}} & reply engagement timestamp & \textit{int}  & timestamp of the Reply engagement if one exists  \\
 & retweet engagement timestamp & \textit{int}  & timestamp of the Retweet engagement if one exists                                  \\
 & quote engagement timestamp & \textit{int}  & timestamp of the Quote engagement if one exists                     \\
  & like engagement timestamp & \textit{int}  & timestamp of the Like engagement if one exists     
  \\
  
  & engageeFollowsEngager    & \textit{bool}                  & Does the account of the engaged tweet author follow the account that                                         \\
                                      &  &                     & has made the engagement?                                         \\ \hline
\end{tabular}

\caption{List of features provided for the challenge dataset}
\label{tab:feature_list}
\end{table}
\end{sidewaystable}


